Cohomology of normic systems and fake Z_p extensions

We set up a general framework to study Tate cohomology groups of Galois modules along $\mathbb{Z}_p$-extensions of number fields. Under suitable assumptions on the Galois modules, we establish the existence of a five-term exact sequence in a certain quotient category whose objects are simultaneously direct and inverse systems, subject to some compatibility. The exact sequence allows one, in particular, to control the behaviour of the Tate cohomology groups of the units along $\mathbb{Z}_p$-extensions. As an application, we study the growth of class numbers along what we call "fake $\mathbb{Z}_p$-extensions of dihedral type". This study relies on a previous work, where we established a class number formula for dihedral extensions in terms of the cohomology groups of the units.

==> CaputoNuccio_NYJM_preamble.tex <==
\usepackage{amsfonts,amsthm,amsmath,amssymb,mathtools}
\usepackage[all,cmtip]{xy}
\usepackage[english]{babel}
\usepackage[utf8]{inputenc}
\usepackage[OT1]{fontenc}
\usepackage{mathrsfs}
\usepackage{xpunctuate}
\usepackage[dvipsnames]{xcolor}
\usepackage{enumitem}
\usepackage[colorlinks=true,linkcolor=Emerald,citecolor=Emerald, backref]{hyperref}  % for hyper-referencing 
\usepackage{geometry}
\numberwithin{equation}{section}
\mathtoolsset{showonlyrefs=true}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem*{theorem*}{Theorem}
\newtheorem*{conjecture}{Conjecture}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem*{defthm*}{Definition/Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem*{lemma*}{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\makeatletter
\newtheorem*{intr@thm}{\intr@thmname}
\newenvironment{introtheorem}[1]{%
	\def\intr@thmname{Theorem #1}
	\begin{intr@thm}}
	{\end{intr@thm}}
\newtheorem*{intr@crl}{\intr@crlname}
\newenvironment{introcorollary}[1]{%
	\def\intr@crlname{Corollary #1}
	\begin{intr@crl}}
	{\end{intr@crl}}
\newtheorem*{intrd@f}{\intrd@fname}
\newenvironment{introdefinition}[1]{%
	\def\intrd@fname{Definition #1}
	\begin{intrd@f}}
	{\end{intrd@f}}
\makeatother


\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
\newtheorem*{acknowledgment}{Acknowledgment}


\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem*{definition*}{Definition}
\newtheorem{assumption}{Assumption}
\newtheorem{notation}[theorem]{Notation}

%%%%%%%%%%%%%%Mathematical symbols
\newcommand{\expp}[1]{p^{#1}}
\newcommand*{\Gal}[2]{\mathrm{Gal}(#1/#2)} % Galois group
\newcommand*{\splitG}[1][0]{D_{#1}} %The extension of \Gamma by \splitG_0
\newcommand*{\filindex}[3][,]{h_{#2#1#3}}
\newcommand*{\subsplit}[1][0]{\Sigma_{#1}} %The subgroup of \splitG isomorphic to \splitG_0
\newcommand*{\catMod}[2][{[\splitG]}]{\mathbf{Mod}^{\mathrm{#2}}_{\ZZ_p#1}} %The category of #1=Z_p[G]-modules, with #2-property.
\newcommand*{\cofg}{co\textrm{-}f.g.} %Property of being co-finitely generated torsion
\newcommand*{\ZZ}{\mathbb{Z}} % rational integers
\newcommand*{\NN}{\mathbb{N}} % positive integers
\newcommand*{\QQ}{\mathbb{Q}} % rational numbers
\DeclareMathOperator{\pr}{pr} %A projection
\makeatletter %%The definition of \cev, a vector going from right to left
\DeclareRobustCommand{\cev}[1]{%
  {\mathpalette\do@cev{#1}}%
}
\newcommand{\do@cev}[2]{%
  \vbox{\offinterlineskip
    \sbox\z@{$\m@th#1 x$}%
    \ialign{##\cr
      \hidewidth\reflectbox{$\m@th#1\vec{}\mkern4mu$}\hidewidth\cr
      \noalign{\kern-\ht\z@}
      $\m@th#1#2$\cr
    }%
  }%
}
\makeatother

%%%%%%%%%%Typical number theoretical objects
\newcommand{\field}[1]{L_{#1}} %the fields in the Z_p-extensions
\newcommand{\rint}[1]{\mathcal{O}_{#1}} % ring of integers
\newcommand{\unit}[1]{\rint{#1}^\times} % units
\newcommand*{\realemb}[1]{r_1(#1)} %number of real embeddings
\newcommand*{\cpxemb}[1]{r_2(#1)} %number of conjugate pairs of complex embeddings
\newcommand{\clgp}[1]{Cl_{#1}} % class group
\newcommand*{\clsyl}[1]{A_{#1}} % p-Sylow of the class group
\newcommand*{\hsyl}[1]{{\varepsilon_{#1}}} % order of the above p-Sylow of the class group
\newcommand*{\algnm}[1]{\mathrm{Nm}_{#1}}% Algebraic norm for the group #1
\newcommand*{\arnm}[2]{\mathrm{N}_{#1/#2}}% Arithmetic norm in the extension #1/#2 (old \nu)
\newcommand*{\arextsymb}{\iota} %The symbol for arrow extension
\newcommand*{\arext}[2]{\arextsymb_{#1/#2}}% Extension of ide(a)l(e)s induced by inclusion of subfields in the extension #1/#2
\newcommand*{\princ}[1]{\mathrm{Pr}_{#1}} % principal ideals
\newcommand*{\ideal}[1]{\mathrm{Id}_{#1}} % ideals
\newcommand*{\aboveT}[1]{\Pi_{#1}} % Classes generated by ramified primes
\newcommand*{\Ram}[2]{\operatorname{T}(#1/#2)} %The primes in #2 which ramify in #1
%\newcommand*{\RamC}[2]{\mathrm{T}'(#1/#2)} %Conjugacy classes of primes in #2 which ramify in #1
\newcommand*{\oram}[2]{\tau(#1/#2)} %The order of the set Ram
\newcommand*{\idele}[1]{\mathbb{A}^\times_{#1}} % ideles
\newcommand*{\idunit}[1]{\mathcal{U}_{#1}} % unit ideles
\newcommand*{\idclg}[1]{\mathcal{C}_{#1}} % ideles class group
\newcommand*{\q}[1]{Q_{#1}} % Schoof's Q
\def\primen@me{p}
\def\conjprimen@me{q}
\def\oth@rprime{l}
\newcommand*{\primeid}{\mathfrak{\primen@me}}
\newcommand*{\conjprimeid}{\mathfrak{\conjprimen@me}}
\newcommand*{\otherprime}{\mathfrak{\oth@rprime}}
\newcommand*{\Primeid}[1]{\mathfrak{\MakeUppercase{\primen@me}}_{#1}}
\newcommand*{\Conjprimeid}[1]{\mathfrak{\MakeUppercase{\conjprimen@me}}_{#1}}
\newcommand*{\Otherprime}[1][\empty]{\mathfrak{\MakeUppercase{\oth@rprime}}_{#1}}
\newcommand*{\locunits}[2][\empty]{\mathbb{E}_{#2}^{#1}} %Local units
\newcommand*{\semiloc}[2][\empty]{\mathcal{V}^{#1}_{#2}} %The semi-local units
\newcommand*{\ramdeg}[2]{e_{#1/#2}} % The ramification index for the _local_ extension (so, no prime needs to be specified) #1/#2
\newcommand*{\indeg}[3][/]{f_{#2#1#3}} % The inertia degree for the _local_ extension (so, no prime needs to be specified) #1/#2
\newcommand*{\logindeg}[1][\empty]{\ell_\infty^{#1}} % The logarithm of the inertia degree for the _local_ Z_p-extension
\newcommand*{\locdeg}[2]{d_{#1/#2}} %The local degree of the local extension #1/#2
\newcommand*{\nprimes}[1][\primeid]{g_{#1}} %Number of primes in L_cyc above #1=\mathfrak{p}
\newcommand*{\fundclass}[2]{u_{#1/#2}} % fundamental class of the extension #1/#2
\newcommand*{\loclev}[1]{E_{#1}} % light notation for the level #1 of the local Z_p-extension
\newcommand*{\invJP}[1][\loclev{\empty}]{\operatorname{inv}_{#1}} %JPS's homomorphism inv

%%%%%%%%%%%%Cohomology%%%%%%%%%%%%%%%
\newcommand{\cch}[1]{\delta^{(#1)}} % cohomological connecting homomorphism H^{#1}(G,C) -> H^{#1 + 1}(G,A) 
\newcommand{\cchT}[1]{\widehat{\delta}^{(#1)}} %The same thing, but leaving from Tate cohomology groups
\newcommand*{\tateiso}[3][\empty]{(\cup\varkappa_{#2}^{#1})^{#3}} % cup product with \chi (#3-#2)/2 times
\DeclarePairedDelimiterXPP{\hh}[3]{\widehat{h}^{#1}}{(}{)}{}{#2,#3} %h^i as order of H^i (both Tate)
\DeclarePairedDelimiterXPP{\hhN}[3]{h^{#1}}{(}{)}{}{#2,#3} %h^i as order of H^i (not Tate)
\DeclarePairedDelimiterXPP{\HH}[3]{\widehat{H}^{#1}}{(}{)}{}{#2,#3} %H^i (Tate)
\DeclarePairedDelimiterXPP{\HHm}[2]{\widehat{H}^{#1}}{(}{)}{}{#2} %H^i (Tate) for a map
\DeclarePairedDelimiterXPP{\HHN}[3]{H^{#1}}{(}{)}{}{#2,#3} %H^i (not Tate) for a module
\DeclareMathOperator{\res}{Res} %res=restriction
\DeclareMathOperator{\defl}{Defl} %Defletion map
\DeclareMathOperator{\infl}{Inf} % Inflation maps
\renewcommand{\inf}{__} % to get an error with AMS definition of inf
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%% Normic and double systems %%%%%%%%%%%
\newcommand*{\pallino}[1][{\field}]{{#1{\bullet}}} %The "bullet" as index for systems. It defaults to L_{\bullet}, but can be modified to be \mathfrak{P}_{\bullet} (setting [1]=[\Primeid]) or p^\bullet (setting [1]=[\expp])
\newcommand*{\nsu}{j} %The "going up" morphism in normic systems
\newcommand*{\nsd}{k} %The "going up" morphism in normic systems
\newcommand*{\normsys}{\mathbf{NS}_{\DD}} %The category of normic systems
\newcommand*{\hatnsu}[2][\jmath]{\widehat{#1}_{#2}} % The "going up" morphism in 0th Tate cohomology of normic systems with surjective going down
\makeatletter
\DeclarePairedDelimiterXPP{\s@sHH}[2]{\p@rH^{#1}}{(}{)}{}{#2} %The double system of H^i (Tate)
\newcommand{\sysHH}[3][\empty]{%
\def\p@rH{\widehat{\calH}_{#1}}
\s@sHH{#2}{#3}%
%\relax
}
\makeatother

\newcommand*{\sysnorm}[1]{\overline{\mathcal{N}#1}} %The double systems of the norms down to F, modulo p^n-th powers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%Other arithmetic operators %%%%%%%%%%%%%%%%
%%The command \roots: called without option, as in \roots{M}, gives \mu_M; with an option, as in \roots[3]{M} gives \mu_M(3)
\makeatletter
\def\r@otsl#1#2#3#4{\mu_{#4}(#2)}
\def\r@ots#1{\mu_{#1}}
\def\roots{\futurelet\radici\r@otschose}
\def\r@otschose{%
	\ifx\radici[
		\expandafter\r@otsl
	\else
		\expandafter\r@ots
\fi}
\makeatother %End of def. for roots
\newcommand{\defect}[2]{\beta_{#1}} % "q-defect" of K, defined as \mu_K/\mu_K^q.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%Iwasawa-theoretic objects %%%%%%%%%%%%%%%%
\newcommand*{\iwLambda}[1][]{\Lambda#1} %The Iwasawa algebra
\newcommand*{\topgen}{\gamma_0} %A topological generator of Gamma
\newcommand*{\iwmu}[2][]{\mu_{#2}^{#1}} % Iwasawa mu
\newcommand*{\iwlambda}[2][]{\lambda_{#2}^{#1}} % Iwasawa lambda
\newcommand*{\lambdacohom}[2][\unit{\pallino}]{\lambda(#2,#1)}
\newcommand*{\iwnu}[2][]{\nu_{#2#1}} % Iwasawa nu 
\makeatletter
\def\th@X{X} % Iwasawa X
\newcommand*{\iwXL}{\th@X_{\iw}} % Iwasawa XL
\newcommand*{\iwXK}{\th@X_{\fk}} % Iwasawa XK
\makeatother
\newcommand*{\indextr}[1][\fromkprimeid]{{n_\mathrm{tr}^{#1}}} %The index starting from which the Zp_extension is totally ramified; either locally or globally
\newcommand*{\Lcyc}{L_\mathrm{cyc}} %The cyclotomic Z_p extension of F
\newcommand*{\Ldue}{\widetilde{L}} %The compositum of Lcyc and Linfty
\newcommand*{\DD}{\mathcal{D}} %The Galois group L_\infty/k
\newcommand*{\GG}{\mathcal{G}} %The Galois group L_\infty/Q
\newcommand*{\Minfty}{M_\infty} %The maximal unramified ext's of the anticyclotomic of F=im.quadratic
\newcommand*{\Frob}[2]{\operatorname{Frob}(#1,#2)} %The Frobenius element at the prime #1 in the extension #2
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%Paper specific%%%%%%%%%
\newcommand*{\nuceta}[1]{\eta_{#1}} %Nuccio's eta
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%Algebraic objects %%%%%%%%%%%%%%%%%
\DeclareMathOperator{\rank}{rk} %rank
\DeclareMathOperator{\corank}{cork} %corank
\DeclarePairedDelimiterX\gindex[2]{(}{)}{#1:#2} % index of a subgroup
\DeclarePairedDelimiter\gorder{\lvert}{\rvert} % order of a group
\renewcommand{\ker}{__} % to get an error with AMS definition of kernel
\newcommand*{\kernel}[1]{\operatorname{Ker} #1} % kernel
\newcommand*{\cokernel}[1]{\operatorname{Coker} #1} % cokernel
\newcommand*{\im}[1]{\operatorname{Im} #1}%image
\newcommand*{\tors}[2][p]{{{#2}[#1]}}%q-torsion
\renewcommand*{\div}[1]{\bigl(#1\bigr)_{\mathrm{div}}} %maximal divisible subgroup
\newcommand*{\id}[1]{\mathrm{id}_{#1}} %identity isomorphism
\DeclareMathOperator{\Hom}{Hom}
\newcommand*{\sch}{\delta} % snake connecting homomorphism
\makeatletter
\newcommand{\Ind}[2]{%
\def\gr@up{#1}%
\def\subgr@up{#2}%
\operatorname{Ind}_{\gr@up}^{\subgr@up} 
					} %Induction from a subgroup
\makeatother

%%%%%%%%Categories%%%%%%%%%%%%%%%
\makeatletter
\newcommand*{\dblsys}[2][\empty]{\mathbf{DS}^{\mathrm{#1}}_{#2}}%_{\ZZ_p}} %Double systems
\newcommand*{\dsu}{\varphi} %The going up morphism for double systems
\newcommand*{\dsd}{\pi}  %The going down morphism for double systems
\newcommand*{\capzero}[2][\scriptscriptstyle\vartriangle]{{^{#1}{#2}}} % Caputo's kernel
\newcommand*{\capbar}[2][\scriptscriptstyle\blacktriangle]{{_{#1}{#2}}} %Caputo's quotient
\newcommand*{\nuczero}[2][\dagger]{{^{#1}{#2}}} %Nuccio's (other) kernel
\newcommand*{\nucbar}[2][\ddagger]{{_{#1}{#2}}} %Nuccio's (other) quotient
\newcommand*{\bddsys}[2][\empty]{\mathbf{B}^{\mathrm{#1}}_{#2}} %Bounded systems for generic \splitG
\newcommand*{\quotsys}[2][\empty]{{\dblsys[#1]{#2}}/{\bddsys[#1]{#2}}} %The quotient category (double)/(bounded)
\newcommand*{\natr}{\Phi} %The natural transformation between id and limemb
\newcommand*{\bddcong}[1][\bddsys{\DD}]{\cong_{#1}} %Isomorphism in the quotient category
\newcommand*{\bddeq}{\propto} %equality up to a bounded error
\newcommand*{\longdashrightarrow}{\dashrightarrow} 
\makeatother
\newcommand*{\stepfunctor}{\mathscr{S}}
\newcommand*{\limemb}{\mathscr{L}} %The composition of varinjlim and \embup
\newcommand*{\calH}{\mathcal{H}}
\newcommand*{\calX}{\mathcal{X}}
\newcommand*{\calY}{\mathcal{Y}}
\newcommand*{\calZ}{\mathcal{Z}}
\newcommand*{\calB}{\mathcal{B}}
\newcommand*{\calC}{\mathcal{C}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%Abreviations and other typography%%%%%%%%%%%%%%
\newcommand*{\longhookrightarrow}{\lhook\joinrel\relbar\joinrel\rightarrow} %Long injective arrow
\newcommand*{\longhookdashedarrow}{\lhook\dashrightarrow} %Long injective dashed arrow
\newcommand*{\longtwoheadrightarrow}{\joinrel\relbar\joinrel\twoheadrightarrow}%Long surjective arrow
\newcommand*{\longtwoheaddashedarrow}{\dashrightarrow\mathrel{\mkern-19mu}\dashrightarrow}%Long surjective dashed arrow
\newcommand{\ie}{\textit{i.~e.~}} % id est
\newcommand*{\rsp}{{resp.~}} % respectively: not \resp to search it in the file
\newcommand{\loccit}{\emph{loc.\kern3pt cit}\xperiod} % loco citato
\newcommand{\ibid}{\emph{ibid}\xperiod} % ibidem
\newcommand{\fk}{\mathrm{fake}} %Roman "fake"
\newcommand{\cyc}{\mathrm{cyc}} %Roman "cyc"
\newcommand{\iw}{\mathrm{Iw}} %For the "classical" Iwasawa invariants
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
